Gated2Depth: Real-time Dense Lidar from Gated Images

We present an imaging framework which converts three images from a gated camera into high-resolution depth maps with depth accuracy comparable to pulsed lidar measurements. Existing scanning lidar systems achieve low spatial resolution at large ranges due to mechanically-limited angular sampling rates, restricting scene understanding tasks to close-range clusters with dense sampling. Moreover, today's pulsed lidar scanners suffer from high cost, power consumption, large form-factors, and they fail in the presence of strong backscatter. We depart from point scanning and demonstrate that it is possible to turn a low-cost CMOS gated imager into a dense depth camera with at least 80m range - by learning depth from three gated images. The proposed architecture exploits semantic context across gated slices, and is trained on a synthetic discriminator loss without the need of dense depth labels. The proposed replacement for scanning lidar systems is real-time, handles back-scatter and provides dense depth at long ranges. We validate our approach in simulation and on real-world data acquired over 4,000km driving in northern Europe. Data and code are available at https://github.com/gruberto/Gated2Depth.

==> fig/results/gta/gta_test_night_example_images.tex <==
\begin{tabular}{ccccccc}
RGB & Full Gated & Lidar & Lidar+RGB  \cite{ma2018sparse} & Gated2Depth & RT Model \cite{adam2017bayesian} & Least Squares \\
\includegraphics[width=0.14285714285714285\textwidth]{figures/results/gta/2018-09-05_20-02-08_0000049723_rgb.jpg} &
\includegraphics[width=0.14285714285714285\textwidth]{figures/results/gta/2018-09-05_20-02-08_0000049723_gated.jpg} &
\includegraphics[width=0.14285714285714285\textwidth]{figures/results/gta/2018-09-05_20-02-08_0000049723_lidar.jpg} &
\includegraphics[width=0.14285714285714285\textwidth]{figures/results/gta/2018-09-05_20-02-08_0000049723_sparse2dense.jpg} &
\includegraphics[width=0.14285714285714285\textwidth]{figures/results/gta/2018-09-05_20-02-08_0000049723_gated2depth.jpg} &
\includegraphics[width=0.14285714285714285\textwidth]{figures/results/gta/2018-09-05_20-02-08_0000049723_baseline_rt_model.jpg} &
\includegraphics[width=0.14285714285714285\textwidth]{figures/results/gta/2018-09-05_20-02-08_0000049723_analytical_ls.jpg}\\
Monocular \cite{Godard2017} & Monocular \cite{Kuznietsov2017} & Mono Gated \cite{Godard2017} & Mono Gated \cite{Kuznietsov2017} & Stereo \cite{Chang2018} & Stereo \cite{pilzer2018unsupervised} &  \\
\includegraphics[width=0.14285714285714285\textwidth]{figures/results/gta/2018-09-05_20-02-08_0000049723_monodepth.jpg} &
\includegraphics[width=0.14285714285714285\textwidth]{figures/results/gta/2018-09-05_20-02-08_0000049723_semodepth.jpg} &
\includegraphics[width=0.14285714285714285\textwidth]{figures/results/gta/2018-09-05_20-02-08_0000049723_monodepth_gated.jpg} &
\includegraphics[width=0.14285714285714285\textwidth]{figures/results/gta/2018-09-05_20-02-08_0000049723_semodepth_gated.jpg} &
\includegraphics[width=0.14285714285714285\textwidth]{figures/results/gta/2018-09-05_20-02-08_0000049723_psm.jpg} &
\includegraphics[width=0.14285714285714285\textwidth]{figures/results/gta/2018-09-05_20-02-08_0000049723_unsup.jpg} &
 \\
\end{tabular}
